Optical and Opto-Mechanical Design of a Novel "Macro" Image Slicer for the MIRADAS Instrument

We present the innovative macro-slicer optical and opto-mechanical designs for the third-generation Mid-resolution InfraReD Astronomical Spectrograph (MIRADAS) instrument for the 10.4m Gran Telescopio Canarias (GTC) in the 1-2.5 $\mu$m bandpass. MIRADAS uses up to 12 cryogenic, fully steerable probes to select simultaneous targets in a 5 arcminute field of view. The spectrograph module is a cross-dispersed echelle spectrograph. The macro-slicer is effectively a stack of six advanced image slicer Integral Field Units (IFUs) such as FRIDA or FISICA, and like other IFUs designed and built at the University of Florida by our group, uses a `bolt-and-go' approach to minimize the difficulty in alignment and maximize robustness. Like other advanced image slicer IFUs, there are three sets of mirrors that work together to geometrically rearrange the loosely packed inputs from the probe arms into a tightly packed pseudo-slit. The macro-slicer also passively keeps the spectral resolution of MIRADAS fixed at $R>20,000$ in seeing from 1.2 arcseconds down to 0.4 arcseconds, (typical observing conditions at GTC).

==> macroSlicerOverview.tex <==
% !TEX root = ./../Stelter_MacroSlicer_SPIE_22March2016.tex

%% 
\small{
\begin{tabularx}{0.625\textwidth}{ccccc}
\toprule
Mirror Block	& \# Mirrors	& Powered? & input f-speed	& output f-speed	\\
\midrule
Beam Combiner	& 12	& No	& ---	& --- 	\\	
Slicer		& 18		& Yes	& 14.2	& ---	\\
Pupil		& 18		& Yes	& ---	& 7.1	\\
Field		& 36		& No	& 7.1	& 7.1	\\
\bottomrule
\end{tabularx}
} % end small
\endinput
%: endinput
%: hg wants a blank line at EOF


==> opticalDescription.tex <==
% !TEX root = ./../Stelter_MacroSlicer_SPIE_22March2016.tex

%% 
\small{
\begin{tabularx}{0.6\textwidth}{cccc}
\toprule
	& F-speed	& Plate Scale	& Pseudo-Slit Length	\\
 	& [unitless]	& [\sfrac{\arcsec}{mm}]	& [mm]  \\
\midrule
Telescope output	& 17.2	& 1.	& --- \\
Probe output		& 14.15	& 1.4575	& \til200 \\
Macro-Slicer output	& 7.10	& 2.9050	& \til 100	\\
\bottomrule
\end{tabularx}
} % end small
\endinput
%: endinput
%: hg wants a blank line at EOF

